Combating Data Laundering in LLM Training

Post-hoc unauthorized-training data detection for large language models (LLMs) typically assumes a query-with-originals regime: rights holders query a target LLM with raw proprietary data and assess whether the model assigns them stronger memorization-based detection signals, e.g., higher confidence or lower loss, than held-out non-training reference texts. We show that this regime becomes brittle under data laundering, where the target LLM is trained on semantics-preserving but stylistically or structurally transformed surrogates of proprietary data to obfuscate provenance. Since training-time exposure occurs in the laundered form, memorization signals may no longer appear on the originals, collapsing the candidate-reference signal separation that standard detectors rely on. We counter this threat by studying laundering-aware detection with raw proprietary data, a held-out reference corpus, and query access to the target LLM, while the laundering transformation is undisclosed. Since exact recovery of the laundered corpus is infeasible, we infer a detection-useful synthesis process via an auxiliary LLM that maps originals into training-like queries. To make this search tractable, we introduce Synthesis Data Reversion (SDR), which constrains the unbounded space of natural-language transformations through a goal-details abstraction: a high-level transformation goal, e.g., "lyrical rewriting", and fine-grained details, e.g., "with vivid imagery". SDR identifies the most likely goal and iteratively refines details so synthesized queries elicit stronger target-model detection signals. Evaluated on the MIMIR benchmark against diverse laundering practices and target LLM families (Pythia, Llama2, and Falcon), SDR consistently restores detection signals, offering a practical auditing layer against data laundering.

==> tables/comparison_existing_survey.tex <==
\begin{table}[b]
\caption{
Comparison with existing surveys related to reprogramming and prompting techniques.
Unlike existing surveys that focus on specific modalities, applications, model architectures, or benchmarks, this work aims to systematically organize the diverse (and sometimes miscellaneous) methodologies and terminologies under a unified conceptual framework with a clear taxonomy. 
}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llllllll}
\toprule
\textbf{Survey Focus} & \citet{gu2023systematic} & \citet{schulhoff2024prompt} & \citet{luo2024incontext} & \citet{zhang2023survey} & \citet{wu2024visual} & \citet{chen2024model} & Ours \\
\midrule
\textbf{In-Modal Progress}                 & \checkmark     & \checkmark        & \checkmark    & \checkmark & \checkmark    &         &      \\
\textbf{Application-targeted}              & \checkmark     & \checkmark        & \checkmark    & \checkmark & \checkmark    &         &      \\
\textbf{Benchmarks}                   &         & \checkmark        &        &     &        &         &      \\
\textbf{Arch-agnostic}          & \checkmark     &            &        &     & \checkmark    & \checkmark     & \checkmark  \\
\textbf{Cross-Field}           &         & \checkmark        &        &     &        &         & \checkmark  \\
\textbf{Unifying Paradigm}        &         &            &        &     &        &         & \checkmark \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/comparison_manifest.tex <==
% \begin{table}[t]
% \centering
% \caption{A comparative analysis of existing RCA literature through the lens of reprogrammability.
% Under interface ($\ell$), setup $\gX^{\rm S}$, $\gE$, and $\gH$ denote manipulations that occur in input space, embedding space, and hidden space, respectively.
% Under configuration ($\lambda$), setup OP and FX means optimizable and fixed manipulations.
% Under operator ($\tau$), setup AD, CO, and TR refers to additive, concatenative, and transformative operators.
% Under mapping ($\omega$), setup SA, LE, RB, and ID represent statistics-based alignment, learning-based alignment, rule-based alignment, and identity mapping.
% }
% \label{tab: framework_manifestation}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{@{}lcccccccccccc@{}}
% \toprule
% & \multicolumn{8}{c}{\textbf{Input Manipulation ($I$)}} & \multicolumn{4}{c}{\textbf{Output Alignment ($O$)}} \\
% \cmidrule(lr){2-9} \cmidrule(lr){10-13}
% & \multicolumn{3}{c}{interface ($\ell$)} & \multicolumn{2}{c}{configuration ($\lambda$)} & \multicolumn{3}{c}{operator ($\tau$)} & \multicolumn{4}{c}{mapping ($\omega$)} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-9} \cmidrule(lr){10-13}
% \textbf{Setup} & $\gX^{\rm S}$ & $\gE$ & $\gH$ & OP & FX & AD & CO & TR & SA & LE & RB & ID \\
% \midrule
% \textbf{MR} & \checkmark & \checkmark &            & \checkmark &            & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &            &            \\
% \textbf{PT} &            & \checkmark & \checkmark & \checkmark &            &            & \checkmark & \checkmark &            & \checkmark & \checkmark & \checkmark \\
% \textbf{PI} & \checkmark &            &            &            & \checkmark & \checkmark & \checkmark & \checkmark &            &            & \checkmark & \checkmark \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
